Data to Physicalization: A Survey of the Physical Rendering Process

Physical representations of data offer physical and spatial ways of looking at, navigating, and interacting with data. While digital fabrication has facilitated the creation of objects with data-driven geometry, rendering data as a physically fabricated object is still a daunting leap for many physicalization designers. Rendering in the scope of this research refers to the back-and-forth process from digital design to digital fabrication and its specific challenges. We developed a corpus of example data physicalizations from research literature and physicalization practice. This survey then unpacks the "rendering" phase of the extended InfoVis pipeline in greater detail through these examples, with the aim of identifying ways that researchers, artists, and industry practitioners "render" physicalizations using digital design and fabrication tools.

==> 9_Table_Taxonomy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[h!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ | p{2cm} | p{2cm} | p{4cm} | p{3cm} | }
\hline
\multirow{10}{=}{Type classification}                      & \multirow{2}{=}{classical type division}        & infovis                                    &                                     \\
                                                           &                                                 & scivis                                     &                                     \\
                                                           & \multirow{2}{=}{intent}                         & pragmatic                                  &                                     \\
                                                           &                                                 & artistic                                   &                                     \\
                                                           & \multirow{3}{=}{technology}                     & passive                                    &                                     \\
                                                           &                                                 & active                                     &                                     \\
                                                           &                                                 & augmented                                  &                                     \\
                                                           & \multirow{3}{=}{application-centric}            & simplifying scientific information         &                                     \\
                                                           &                                                 & educational tools                          &                                     \\
                                                           &                                                 & didactic installations                     &                                     \\ \cline{2-3}
\multirow{20}{=}{target data and visual encoding}          & \multirow{10}{=}{datasets and data types}       & biological                                 &                                     \\ 
                                                           &                                                 & medical                                    &                                     \\ 
                                                           &                                                 & mathematical                               &                                     \\ 
                                                           &                                                 & personal and activity data                 &                                     \\ 
                                                           &                                                 & geospatial                                 &                                     \\ 
                                                           &                                                 & image/video used as data                   &                                     \\ 
                                                           &                                                 & country indicators                         &                                     \\ 
                                                           &                                                 & statistical                                &                                     \\ 
                                                           &                                                 & environmental                              &                                     \\ 
                                                           &                                                 & other                                      &                                     \\ \cline{3-3}
                                                           & \multirow{4}{=}{data collection and processing} & through observation                        &                                     \\
                                                           &                                                 & governmental data                          &                                     \\
                                                           &                                                 & institutional data                         &                                     \\
                                                           &                                                 & qualitative data collection                &                                     \\ \cline{3-3}
                                                           & \multirow{6}{=}{visual encoding idiom}          & 3D physical charts                         &                                     \\
                                                           &                                                 & topography and physical elevantion models  &                                     \\
                                                           &                                                 & architectural spaces (data spatialization) &                                     \\
                                                           &                                                 & landscape models                           &                                     \\
                                                           &                                                 & biological and molecular models            &                                     \\
                                                           &                                                 & objects with no graphical precedents       &                                     \\ \cline{2-3}
\multirow{25}{=}{design and physical rendering approaches} & \multirow{6}{=}{digital design}                 & 2D CAD                                     &                                     \\ \cline{4-4}
                                                           &                                                 & \multirow{3}{=}{3D CAD}                    & polygonal meshes                    \\
                                                           &                                                 &                                            & NURBS                               \\
                                                           &                                                 &                                            & OpenSCAD                            \\ \cline{4-4}
                                                           &                                                 & Algorithmic and parametric design          &                                     \\
                                                           &                                                 & CAD by programming                         &                                     \\
                                                           & \multirow{2}{=}{Augmentation design approaches} & projection augmentation                    &                                     \\
                                                           &                                                 & augmentation through augmented reality     &                                     \\ \cline{3-3}
                                                           & \multirow{8}{=}{Digital fabrication}            & 2D printing                                &                                     \\ \cline{4-4}
                                                           &                                                 &  \multirow{2}{=}{additive techniques}       & FDM 3D printing                     \\
                                                           &                                                 &                                            & layer solidification 3D printing    \\ \cline{4-4}
                                                           &                                                 &  \multirow{2}{=}{subtractive techniques}    & CNC                                 \\
                                                           &                                                 &                                            & cutting techniques                  \\ \cline{4-4}
                                                           &                                                 & formative techniques                       &                                     \\
                                                           &                                                 & hybrid fabrication techniques              &                                     \\
                                                           &                                                 & manual assembly                            &                                     \\ \cline{3-4}
                                                           & \multirow{8}{=}{active rendering techniques}    & \multirow{2}{=}{goals}                     & changing a single dataset           \\
                                                           &                                                 &                                            & supporting multiple dataset         \\ \cline{4-4}
                                                           &                                                 & \multirow{4}{=}{active physical platforms} & shape changing displays             \\
                                                           &                                                 &                                            & deformable surfaces                 \\
                                                           &                                                 &                                            & small robots                        \\
                                                           &                                                 &                                            & robotic arm                         \\ \cline{4-4}
                                                           &                                                 & \multirow{2}{=}{movement implementation}   & microprocessor type and programming \\
                                                           &                                                 &                                            & parts to support movements          \\ \cline{3-4}
                                                           & automated physical rendering techniques         &                                            &    \\                                
\hline
\end{tabular}
}
\caption{Overview of the taxonomy presented in \autoref{sec:classification} to \autoref{sec:rendering}.}
\label{tab:taxonomyOverview}
\end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

